Memory and Resource Leak Defects and their Repairs in Java Projects

Despite huge software engineering efforts and programming language support, resource and memory leaks are still a troublesome issue, even in memory-managed languages such as Java. Understanding the properties of leak-inducing defects, how the leaks manifest, and how they are repaired is an essential prerequisite for designing better approaches for avoidance, diagnosis, and repair of leak-related bugs. We conduct a detailed empirical study on 491 issues from 15 large open-source Java projects. The study proposes taxonomies for the leak types, for the defects causing them, and for the repair actions. We investigate, under several aspects, the distributions within each taxonomy and the relationships between them. We find that manual code inspection and manual runtime detection are still the main methods for leak detection. We find that most of the errors manifest on error-free execution paths, and developers repair the leak defects in a shorter time than non-leak defects. We also identify 13 recurring code transformations in the repair patches. Based on our findings, we draw a variety of implications on how developers can avoid, detect, isolate and repair leak-related bugs.

==> ref <==
\begin{thebibliography}{68}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{DOI~\discretionary{}{}{}#1}\else
  \providecommand{\doi}{DOI~\discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url}\fi
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem[{plu(2017)}]{plumbr}
 (2017) Plumbr. \url{https://plumbr.eu/blog}, accessed: 2017-02-01

\bibitem[{Artstein and Poesio(2008)}]{KappaLinguistics}
Artstein R, Poesio M (2008) Inter-coder agreement for computational
  linguistics. Comput Linguist 34(4):555--596, \doi{10.1162/coli.07-034-R2},
  \urlprefix\url{http://dx.doi.org/10.1162/coli.07-034-R2}

\bibitem[{Banerjee et~al.(2018)Banerjee, Chong, Ballabriga, and
  Roychoudhury}]{androidResourceLeakEnergy}
Banerjee A, Chong LK, Ballabriga C, Roychoudhury A (2018) Energypatch:
  Repairing resource leaks to improve energy-efficiency of android apps. IEEE
  Transactions on Software Engineering 44(5):470--490,
  \doi{10.1109/TSE.2017.2689012},
  \urlprefix\url{doi.ieeecomputersociety.org/10.1109/TSE.2017.2689012}

\bibitem[{Bond and McKinley(2006)}]{BellLeak2006}
Bond MD, McKinley KS (2006) Bell: Bit-encoding online memory leak detection.
  In: Proceedings of the 12th International Conference on Architectural Support
  for Programming Languages and Operating Systems, ASPLOS XII, pp 61--72,
  \doi{10.1145/1168857.1168866},
  \urlprefix\url{http://doi.acm.org/10.1145/1168857.1168866}

\bibitem[{Bond and McKinley(2008)}]{ToleratingLeak}
Bond MD, McKinley KS (2008) Tolerating memory leaks. In: Proceedings of the
  23rd ACM SIGPLAN Conference on Object-oriented Programming Systems Languages
  and Applications, OOPSLA '08, pp 109--126, \doi{10.1145/1449764.1449774},
  \urlprefix\url{http://doi.acm.org/10.1145/1449764.1449774}

\bibitem[{Bond and McKinley(2009)}]{LeakPruningBond2009}
Bond MD, McKinley KS (2009) Leak pruning. In: ACM Conference on Architectural
  Support for Programming Languages and Operating Systems (ASPLOS), ASPLOS XIV,
  pp 277--288, \doi{10.1145/1508244.1508277},
  \urlprefix\url{http://doi.acm.org/10.1145/1508244.1508277}

\bibitem[{Chen et~al.(2016)Chen, Shang, Yang, Hassan, Godfrey, Nasser, and
  Flora}]{ORMEntropy}
Chen TH, Shang W, Yang J, Hassan AE, Godfrey MW, Nasser M, Flora P (2016) An
  empirical study on the practice of maintaining object-relational mapping code
  in java systems. In: Proceedings of the 13th International Conference on
  Mining Software Repositories, ACM, MSR '16, pp 165--176,
  \doi{10.1145/2901739.2901758},
  \urlprefix\url{http://doi.acm.org/10.1145/2901739.2901758}

\bibitem[{Cherem and Rugina(2004)}]{CheremResourceLeak}
Cherem S, Rugina R (2004) Region analysis and transformation for java programs.
  In: Proceedings of the 4th International Symposium on Memory Management, ISMM
  '04, pp 85--96, \doi{10.1145/1029873.1029884},
  \urlprefix\url{http://doi.acm.org/10.1145/1029873.1029884}

\bibitem[{Cherem et~al.(2007)Cherem, Princehouse, and Rugina}]{Cheremleak2007}
Cherem S, Princehouse L, Rugina R (2007) Practical memory leak detection using
  guarded value-flow analysis. In: Proceedings of the 2007 ACM SIGPLAN
  Conference on Programming Language Design and Implementation, PLDI '07, pp
  480--491, \doi{10.1145/1250734.1250789},
  \urlprefix\url{http://doi.acm.org/10.1145/1250734.1250789}

\bibitem[{Clause and Orso(2010)}]{leakpoint}
Clause J, Orso A (2010) Leakpoint: Pinpointing the causes of memory leaks. In:
  Proceedings of the 32Nd ACM/IEEE International Conference on Software
  Engineering - Volume 1, ICSE '10, pp 515--524, \doi{10.1145/1806799.1806874},
  \urlprefix\url{http://doi.acm.org/10.1145/1806799.1806874}

\bibitem[{Cohen(1960)}]{kappaCohen}
Cohen J (1960) A coefficient of agreement for nominal scales. Educational and
  Psychological Measurement 20(1):37--46, \doi{10.1177/001316446002000104},
  \urlprefix\url{https://doi.org/10.1177/001316446002000104},
  \eprint{https://doi.org/10.1177/001316446002000104}

\bibitem[{Dillig et~al.(2008)Dillig, Dillig, Yahav, and
  Chandra}]{CloserResourceLeak}
Dillig I, Dillig T, Yahav E, Chandra S (2008) The closer: Automating resource
  management in java. In: ACM International Symposium on Memory Management
  (ISMM), pp 1--10, \doi{10.1145/1375634.1375636},
  \urlprefix\url{http://doi.acm.org/10.1145/1375634.1375636}

\bibitem[{Fang et~al.(2015)Fang, Dou, and Xu}]{perfblower}
Fang L, Dou L, Xu GH (2015) Perfblower: Quickly detecting memory-related
  performance problems via amplification. In: 29th European Conference on
  Object-Oriented Programming, {ECOOP} 2015, July 5-10, 2015, Prague, Czech
  Republic, pp 296--320, \doi{10.4230/LIPIcs.ECOOP.2015.296},
  \urlprefix\url{http://dx.doi.org/10.4230/LIPIcs.ECOOP.2015.296}

\bibitem[{Gao et~al.(2015)Gao, Xiong, Mi, Zhang, Yang, Zhou, Xie, and
  Mei}]{SafeLeakFixC}
Gao Q, Xiong Y, Mi Y, Zhang L, Yang W, Zhou Z, Xie B, Mei H (2015) Safe
  memory-leak fixing for c programs. In: Proceedings of the 37th International
  Conference on Software Engineering - Volume 1, ICSE '15, pp 459--470,
  \urlprefix\url{http://dl.acm.org/citation.cfm?id=2818754.2818812}

\bibitem[{Ghanavati and Andrzejak(2015)}]{SCAM2015}
Ghanavati M, Andrzejak A (2015) Automated memory leak diagnosis by regression
  testing. In: 2015 IEEE 15th International Working Conference on Source Code
  Analysis and Manipulation (SCAM), pp 191--200,
  \doi{10.1109/SCAM.2015.7335415}

\bibitem[{Ghanavati et~al.(2018)Ghanavati, Costa, Andrzejak, and
  Seboek}]{PosterICSE2018}
Ghanavati M, Costa D, Andrzejak A, Seboek J (2018) Memory and resource leak
  defects in java projects: An empirical study. In: Proceedings of the 38th
  International Conference on Software Engineering Companion, ICSE '18
  Companion, pp 410--411, \doi{10.1145/3183440.3195032},
  \urlprefix\url{https://doi.org/10.1145/3183440.3195032}

\bibitem[{Guo et~al.(2013)Guo, Zhang, Yan, Zhang, and
  Zhang}]{androidResourceLeak}
Guo C, Zhang J, Yan J, Zhang Z, Zhang Y (2013) Characterizing and detecting
  resource leaks in android applications. In: Proceedings of the 28th IEEE/ACM
  International Conference on Automated Software Engineering, IEEE Press,
  Piscataway, NJ, USA, ASE'13, pp 389--398, \doi{10.1109/ASE.2013.6693097},
  \urlprefix\url{https://doi.org/10.1109/ASE.2013.6693097}

\bibitem[{Hassan(2009)}]{entropyHassan}
Hassan AE (2009) Predicting faults using the complexity of code changes. In:
  Proceedings of the 31st International Conference on Software Engineering,
  IEEE Computer Society, ICSE '09, pp 78--88, \doi{10.1109/ICSE.2009.5070510},
  \urlprefix\url{http://dx.doi.org/10.1109/ICSE.2009.5070510}

\bibitem[{Hauswirth and Chilimbi(2004)}]{SWATLeak2004}
Hauswirth M, Chilimbi TM (2004) Low-overhead memory leak detection using
  adaptive statistical profiling. In: Proceedings of the 11th International
  Conference on Architectural Support for Programming Languages and Operating
  Systems, ASPLOS XI, pp 156--164, \doi{10.1145/1024393.1024412},
  \urlprefix\url{http://doi.acm.org/10.1145/1024393.1024412}

\bibitem[{Heine and Lam(2003)}]{HeineCLeak2003}
Heine DL, Lam MS (2003) A practical flow-sensitive and context-sensitive c and
  c++ memory leak detector. In: Proceedings of the ACM SIGPLAN 2003 Conference
  on Programming Language Design and Implementation, PLDI '03, pp 168--181,
  \doi{10.1145/781131.781150},
  \urlprefix\url{http://doi.acm.org/10.1145/781131.781150}

\bibitem[{Huizinga and Kolawa(2007)}]{BestPractices}
Huizinga D, Kolawa A (2007) Automated defect prevention: best practices in
  software management. John Wiley \& Sons, USA

\bibitem[{Humphrey(2000)}]{PSP2000}
Humphrey W (2000) The personal software process (psp). Tech. Rep.
  CMU/SEI-2000-TR-022, Software Engineering Institute, Carnegie Mellon
  University, Pittsburgh, PA,
  \urlprefix\url{http://resources.sei.cmu.edu/library/asset-view.cfm?AssetID=5283}

\bibitem[{Jin et~al.(2012{\natexlab{a}})Jin, Song, Shi, Scherpelz, and
  Lu}]{EmprunderstandingPerfBugs}
Jin G, Song L, Shi X, Scherpelz J, Lu S (2012{\natexlab{a}}) Understanding and
  detecting real-world performance bugs. In: Proceedings of the 33rd ACM
  SIGPLAN Conference on Programming Language Design and Implementation, PLDI
  '12, pp 77--88, \doi{10.1145/2254064.2254075},
  \urlprefix\url{http://doi.acm.org/10.1145/2254064.2254075}

\bibitem[{Jin et~al.(2012{\natexlab{b}})Jin, Song, Shi, Scherpelz, and
  Lu}]{PerfEmprUnderstand}
Jin G, Song L, Shi X, Scherpelz J, Lu S (2012{\natexlab{b}}) Understanding and
  detecting real-world performance bugs. In: Proceedings of the 33rd ACM
  SIGPLAN Conference on Programming Language Design and Implementation, PLDI
  '12, pp 77--88, \doi{10.1145/2254064.2254075},
  \urlprefix\url{http://doi.acm.org/10.1145/2254064.2254075}

\bibitem[{Jump and McKinley(2007)}]{CorkLeak2007}
Jump M, McKinley KS (2007) Cork: Dynamic memory leak detection for
  garbage-collected languages. In: ACM SIGPLAN-SIGACT Symposium on Principles
  of Programming Languages (POPL), pp 31--38, \doi{10.1145/1190216.1190224},
  \urlprefix\url{http://doi.acm.org/10.1145/1190216.1190224}

\bibitem[{Jung et~al.(2014)Jung, Lee, Raman, and Pande}]{leakProduction}
Jung C, Lee S, Raman E, Pande S (2014) Automated memory leak detection for
  production use. In: Proceedings of the 36th International Conference on
  Software Engineering, ICSE 2014, pp 825--836, \doi{10.1145/2568225.2568311},
  \urlprefix\url{http://doi.acm.org/10.1145/2568225.2568311}

\bibitem[{Kim et~al.(2013)Kim, Nam, Song, and Kim}]{templateFix}
Kim D, Nam J, Song J, Kim S (2013) Automatic patch generation learned from
  human-written patches. In: Proceedings of the 2013 International Conference
  on Software Engineering, ICSE '13, pp 802--811,
  \urlprefix\url{http://dl.acm.org/citation.cfm?id=2486788.2486893}

\bibitem[{Langner and Andrzejak(2013)}]{VC2012}
Langner F, Andrzejak A (2013) Detecting software aging in a cloud computing
  framework by comparing development versions. In: IFIP/IEEE Symposium on
  Integrated Network and Service Management (IM), pp 896--899

\bibitem[{Le et~al.(2016)Le, Lo, and Le~Goues}]{HDRepair}
Le XBD, Lo D, Le~Goues C (2016) History driven program repair. In: IEEE 23rd
  International Conference on Software Analysis, Evolution and Reengineering,
  IEEE, SANER '16

\bibitem[{Liu et~al.(2013)Liu, Yang, Tan, and Hafiz}]{R2Fix}
Liu C, Yang J, Tan L, Hafiz M (2013) R2fix: Automatically generating bug fixes
  from bug reports. In: Proceedings of the 2013 IEEE Sixth International
  Conference on Software Testing, Verification and Validation, ICST '13, pp
  282--291, \doi{10.1109/ICST.2013.24},
  \urlprefix\url{https://doi.org/10.1109/ICST.2013.24}

\bibitem[{Lo et~al.(2015)Lo, Nagappan, and Zimmermann}]{LoPractitioners}
Lo D, Nagappan N, Zimmermann T (2015) How practitioners perceive the relevance
  of software engineering research. In: Proceedings of the 2015 10th Joint
  Meeting on Foundations of Software Engineering, ACM, New York, NY, USA,
  ESEC/FSE 2015, pp 415--425, \doi{10.1145/2786805.2786809},
  \urlprefix\url{http://doi.acm.org/10.1145/2786805.2786809}

\bibitem[{Long and Rinard(2016)}]{Prophet}
Long F, Rinard M (2016) Automatic patch generation by learning correct code.
  In: Proceedings of the 43rd Annual ACM SIGPLAN-SIGACT Symposium on Principles
  of Programming Languages, POPL '16, pp 298--312,
  \doi{10.1145/2837614.2837617},
  \urlprefix\url{http://doi.acm.org/10.1145/2837614.2837617}

\bibitem[{Machida et~al.(2012)Machida, Xiang, Tadano, and Maeno}]{fumio}
Machida F, Xiang J, Tadano K, Maeno Y (2012) Aging-related bugs in cloud
  computing software. In: Proceedings of the 2012 IEEE 23rd International
  Symposium on Software Reliability Engineering Workshops, ISSREW '12, pp
  287--292, \doi{10.1109/ISSREW.2012.97},
  \urlprefix\url{http://dx.doi.org/10.1109/ISSREW.2012.97}

\bibitem[{Matias et~al.(2014)Matias, Andrzejak, Machida, Elias, and
  Trivedi}]{Matias_SysDiffAnalysis2014}
Matias R, Andrzejak A, Machida F, Elias D, Trivedi K (2014) A systematic
  differential analysis for fast and robust detection of software aging. In:
  2014 IEEE 33rd International Symposium on Reliable Distributed Systems, pp
  311--320, \doi{10.1109/SRDS.2014.38}

\bibitem[{McConnell(1993)}]{McConnellCodeComplete}
McConnell S (1993) Code complete: a practical handbook of software
  construction. Microsoft Press, USA

\bibitem[{Mechtaev et~al.(2016)Mechtaev, Yi, and Roychoudhury}]{angelix}
Mechtaev S, Yi J, Roychoudhury A (2016) Angelix: Scalable multiline program
  patch synthesis via symbolic analysis. In: Proceedings of the 38th
  International Conference on Software Engineering, ICSE '16, pp 691--701,
  \doi{10.1145/2884781.2884807},
  \urlprefix\url{http://doi.acm.org/10.1145/2884781.2884807}

\bibitem[{Meng et~al.(2013)Meng, Kim, and McKinley}]{LASEPatchGeneration}
Meng N, Kim M, McKinley KS (2013) Lase: Locating and applying systematic edits
  by learning from examples. In: Proceedings of the 2013 International
  Conference on Software Engineering, IEEE Press, Piscataway, NJ, USA, ICSE
  '13, pp 502--511,
  \urlprefix\url{http://dl.acm.org/citation.cfm?id=2486788.2486855}

\bibitem[{Mitchell and Sevitsky(2003)}]{Leakbot2003}
Mitchell N, Sevitsky G (2003) Leakbot: An automated and lightweight tool for
  diagnosing memory leaks in large java applications. In: ECOOP 2003 --
  Object-Oriented Programming, pp 351--377

\bibitem[{Nguyen et~al.(2013)Nguyen, Qi, Roychoudhury, and Chandra}]{semfix}
Nguyen HDT, Qi D, Roychoudhury A, Chandra S (2013) Semfix: Program repair via
  semantic analysis. In: Proceedings of the 2013 International Conference on
  Software Engineering, ICSE '13, pp 772--781,
  \urlprefix\url{http://dl.acm.org/citation.cfm?id=2486788.2486890}

\bibitem[{Nguyen et~al.(2015)Nguyen, Wang, Bu, Fang, Hu, and Xu}]{facade}
Nguyen K, Wang K, Bu Y, Fang L, Hu J, Xu G (2015) Facade: A compiler and
  runtime for (almost) object-bounded big data applications. In: Proceedings of
  the Twentieth International Conference on Architectural Support for
  Programming Languages and Operating Systems, ASPLOS '15, pp 675--690

\bibitem[{Nistor et~al.(2013)Nistor, Jiang, and Tan}]{EmprPerfBugMSR}
Nistor A, Jiang T, Tan L (2013) Discovering, reporting, and fixing performance
  bugs. In: Proceedings of the 10th Working Conference on Mining Software
  Repositories, MSR '13, pp 237--246,
  \urlprefix\url{http://dl.acm.org/citation.cfm?id=2487085.2487134}

\bibitem[{Novark et~al.(2009)Novark, Berger, and Zorn}]{HoundLeak2009}
Novark G, Berger ED, Zorn BG (2009) Efficiently and precisely locating memory
  leaks and bloat. In: Proceedings of the 2009 ACM SIGPLAN Conference on
  Programming Language Design and Implementation, PLDI '09, pp 397--407,
  \doi{10.1145/1542476.1542521},
  \urlprefix\url{http://doi.acm.org/10.1145/1542476.1542521}

\bibitem[{Orlovich and Rugina(2006)}]{OrlovichLeak2006}
Orlovich M, Rugina R (2006) Memory leak analysis by contradiction. In:
  Proceedings of the 13th International Conference on Static Analysis, SAS'06,
  pp 405--424, \doi{10.1007/11823230_26},
  \urlprefix\url{http://dx.doi.org/10.1007/11823230_26}

\bibitem[{Pan et~al.(2009)Pan, Kim, and Whitehead}]{27bugPatterns}
Pan K, Kim S, Whitehead EJ Jr (2009) Toward an understanding of bug fix
  patterns. Empirical Softw Engg 14(3):286--315,
  \doi{10.1007/s10664-008-9077-5},
  \urlprefix\url{http://dx.doi.org/10.1007/s10664-008-9077-5}

\bibitem[{Rayside and Mendel(2007)}]{OwnershipProfilingLeak2007}
Rayside D, Mendel L (2007) Object ownership profiling: A technique for finding
  and fixing memory leaks. In: Proceedings of the Twenty-second IEEE/ACM
  International Conference on Automated Software Engineering, ASE '07, pp
  194--203

\bibitem[{Seaman(1999)}]{Seaman99-coding}
Seaman CB (1999) Qualitative methods in empirical studies of software
  engineering. IEEE Trans Softw Eng 25(4):557--572, \doi{10.1109/32.799955},
  \urlprefix\url{http://dx.doi.org/10.1109/32.799955}

\bibitem[{Seaman et~al.(2008)Seaman, Shull, Regardie, Elbert, Feldmann, Guo,
  and Godfrey}]{Seaman2008-coding}
Seaman CB, Shull F, Regardie M, Elbert D, Feldmann RL, Guo Y, Godfrey S (2008)
  Defect categorization: Making use of a decade of widely varying historical
  data. In: Proceedings of the Second ACM-IEEE International Symposium on
  Empirical Software Engineering and Measurement, ESEM '08, pp 149--157,
  \doi{10.1145/1414004.1414030},
  \urlprefix\url{http://doi.acm.org/10.1145/1414004.1414030}

\bibitem[{Selakovic and Pradel(2016)}]{JSPerformance}
Selakovic M, Pradel M (2016) Performance issues and optimizations in
  javascript: An empirical study. In: Proceedings of the 38th International
  Conference on Software Engineering, ACM, New York, NY, USA, ICSE '16, pp
  61--72, \doi{10.1145/2884781.2884829},
  \urlprefix\url{http://doi.acm.org/10.1145/2884781.2884829}

\bibitem[{Shaham et~al.(2003)Shaham, Yahav, Kolodner, and
  Sagiv}]{HeapSafteyLeak}
Shaham R, Yahav E, Kolodner EK, Sagiv M (2003) Establishing local temporal heap
  safety properties with applications to compile-time memory management. In:
  Proceedings of the 10th International Conference on Static Analysis, SAS'03,
  pp 483--503,
  \urlprefix\url{http://dl.acm.org/citation.cfm?id=1760267.1760304}

\bibitem[{Sommerville(2010)}]{SommervilleSoftEng}
Sommerville I (2010) Software Engineering, 9th edn. Addison-Wesley Publishing
  Company, USA

\bibitem[{Song and Lu(2014)}]{EmpPerfStat}
Song L, Lu S (2014) Statistical debugging for real-world performance problems.
  In: Proceedings of the 2014 ACM International Conference on Object Oriented
  Programming Systems Languages \& Applications, OOPSLA '14, pp 561--578,
  \doi{10.1145/2660193.2660234},
  \urlprefix\url{http://doi.acm.org/10.1145/2660193.2660234}

\bibitem[{Sor et~al.(2013)Sor, Oü, Treier, and Srirama}]{sor}
Sor V, Oü P, Treier T, Srirama SN (2013) Improving statistical approach for
  memory leak detection using machine learning. In: 2013 IEEE International
  Conference on Software Maintenance, pp 544--547, \doi{10.1109/ICSM.2013.92}

\bibitem[{Tan et~al.(2014)Tan, Liu, Li, Wang, Zhou, and Zhai}]{bugStudyOpenSrc}
Tan L, Liu C, Li Z, Wang X, Zhou Y, Zhai C (2014) Bug characteristics in open
  source software. Empirical Softw Engg 19(6):1665--1705,
  \doi{10.1007/s10664-013-9258-8},
  \urlprefix\url{http://dx.doi.org/10.1007/s10664-013-9258-8}

\bibitem[{van Tonder and Goues(2018)}]{staticRepairInfer}
van Tonder R, Goues CL (2018) Static automated program repair for heap
  properties. In: Proceedings of the 40th International Conference on Software
  Engineering, ACM, New York, NY, USA, ICSE '18, pp 151--162,
  \doi{10.1145/3180155.3180250},
  \urlprefix\url{http://doi.acm.org/10.1145/3180155.3180250}

\bibitem[{Torlak and Chandra(2010)}]{trackerResourceLeak}
Torlak E, Chandra S (2010) Effective interprocedural resource leak detection.
  In: Proceedings of the 32Nd ACM/IEEE International Conference on Software
  Engineering - Volume 1, ICSE '10, pp 535--544, \doi{10.1145/1806799.1806876},
  \urlprefix\url{http://doi.acm.org/10.1145/1806799.1806876}

\bibitem[{Weimer and Necula(2004)}]{weimarErrrorHandling}
Weimer W, Necula GC (2004) Finding and preventing run-time error handling
  mistakes. In: Proceedings of the 19th Annual ACM SIGPLAN Conference on
  Object-oriented Programming, Systems, Languages, and Applications, ACM, New
  York, NY, USA, OOPSLA '04, pp 419--431, \doi{10.1145/1028976.1029011},
  \urlprefix\url{http://doi.acm.org/10.1145/1028976.1029011}

\bibitem[{Weimer and Necula(2005)}]{weimarTemporalSpecError}
Weimer W, Necula GC (2005) Mining temporal specifications for error detection.
  In: Proceedings of the 11th International Conference on Tools and Algorithms
  for the Construction and Analysis of Systems, Springer-Verlag, Berlin,
  Heidelberg, TACAS'05, pp 461--476, \doi{10.1007/978-3-540-31980-1_30},
  \urlprefix\url{http://dx.doi.org/10.1007/978-3-540-31980-1_30}

\bibitem[{Weimer et~al.(2009)Weimer, Nguyen, Le~Goues, and Forrest}]{genprog}
Weimer W, Nguyen T, Le~Goues C, Forrest S (2009) Automatically finding patches
  using genetic programming. In: Proceedings of the 31st International
  Conference on Software Engineering, ICSE '09, pp 364--374,
  \doi{10.1109/ICSE.2009.5070536},
  \urlprefix\url{http://dx.doi.org/10.1109/ICSE.2009.5070536}

\bibitem[{Wu et~al.(2011)Wu, Zhang, Kim, and Cheung}]{Wu_Relink}
Wu R, Zhang H, Kim S, Cheung SC (2011) Relink: Recovering links between bugs
  and changes. In: Proceedings of the 19th ACM SIGSOFT Symposium and the 13th
  European Conference on Foundations of Software Engineering, ESEC/FSE '11, pp
  15--25, \doi{10.1145/2025113.2025120},
  \urlprefix\url{http://doi.acm.org/10.1145/2025113.2025120}

\bibitem[{Xie and Aiken(2005)}]{XieContextLeakStatic2005}
Xie Y, Aiken A (2005) Context- and path-sensitive memory leak detection. In:
  Proceedings of the 10th European Software Engineering Conference Held Jointly
  with 13th ACM SIGSOFT International Symposium on Foundations of Software
  Engineering, ESEC/FSE-13, pp 115--125, \doi{10.1145/1081706.1081728},
  \urlprefix\url{http://doi.acm.org/10.1145/1081706.1081728}

\bibitem[{Xu and Rountev(2008)}]{leakContainerXu2008}
Xu G, Rountev A (2008) Precise memory leak detection for java software using
  container profiling. In: Proceedings of the 30th International Conference on
  Software Engineering, ICSE '08, pp 151--160, \doi{10.1145/1368088.1368110},
  \urlprefix\url{http://doi.acm.org/10.1145/1368088.1368110}

\bibitem[{Xu and Rountev(2013)}]{leakcontainer2013}
Xu G, Rountev A (2013) Precise memory leak detection for java software using
  container profiling. ACM Trans Softw Eng Methodol 22(3):17:1--17:28,
  \doi{10.1145/2491509.2491511}

\bibitem[{Xu et~al.(2010)Xu, Mitchell, Arnold, Rountev, and
  Sevitsky}]{BloatLeakAnalysis-Xu:2010}
Xu G, Mitchell N, Arnold M, Rountev A, Sevitsky G (2010) Software bloat
  analysis: Finding, removing, and preventing performance problems in modern
  large-scale object-oriented applications. In: FSE/SDP Workshop on Future of
  Software Engineering Research (FoSER), pp 421--426,
  \doi{10.1145/1882362.1882448},
  \urlprefix\url{http://doi.acm.org/10.1145/1882362.1882448}

\bibitem[{Xu et~al.(2011)Xu, Bond, Qin, and Rountev}]{leakchaser}
Xu G, Bond MD, Qin F, Rountev A (2011) Leakchaser: Helping programmers narrow
  down causes of memory leaks. In: Proceedings of the 32Nd ACM SIGPLAN
  Conference on Programming Language Design and Implementation, PLDI '11, pp
  270--282, \doi{10.1145/1993498.1993530},
  \urlprefix\url{http://doi.acm.org/10.1145/1993498.1993530}

\bibitem[{Yan et~al.(2014)Yan, Xu, Yang, and Rountev}]{LeakChecker2014}
Yan D, Xu G, Yang S, Rountev A (2014) Leakchecker: Practical static memory leak
  detection for managed languages. In: Proceedings of Annual IEEE/ACM
  International Symposium on Code Generation and Optimization, CGO '14, pp
  87:87--87:97, \doi{10.1145/2544137.2544151},
  \urlprefix\url{http://doi.acm.org/10.1145/2544137.2544151}

\bibitem[{Yan et~al.(2016)Yan, Sui, Chen, and Xue}]{valueFlowLeakFixC}
Yan H, Sui Y, Chen S, Xue J (2016) Automated memory leak fixing on value-flow
  slices for c programs. In: Proceedings of the 31st Annual ACM Symposium on
  Applied Computing, SAC '16, pp 1386--1393, \doi{10.1145/2851613.2851773},
  \urlprefix\url{http://doi.acm.org/10.1145/2851613.2851773}

\bibitem[{Yin et~al.(2011)Yin, Yuan, Zhou, Pasupathy, and
  Bairavasundaram}]{fixBecomeBug}
Yin Z, Yuan D, Zhou Y, Pasupathy S, Bairavasundaram L (2011) How do fixes
  become bugs? In: Proceedings of the 19th ACM SIGSOFT Symposium and the 13th
  European Conference on Foundations of Software Engineering, ACM, New York,
  NY, USA, ESEC/FSE '11, pp 26--36, \doi{10.1145/2025113.2025121},
  \urlprefix\url{http://doi.acm.org/10.1145/2025113.2025121}

\bibitem[{Zhong and Su(2015)}]{EmprBugFix}
Zhong H, Su Z (2015) An empirical study on real bug fixes. In: Proceedings of
  the 37th International Conference on Software Engineering - Volume 1, ICSE
  '15, pp 913--923,
  \urlprefix\url{http://dl.acm.org/citation.cfm?id=2818754.2818864}

\end{thebibliography}


==> tables/table_action_patterns_correlation.tex <==
\begin{table*}[t]
\centering
\caption{A taxonomy of common code transformations and the repair actions using these transformations. 
%The numbers in parentheses in Column ``Repair Actions'' show the frequency of code transformation for each repair action.
}
\begin{tabular}{lll}
%\begin{tabular}{p{2cm}p{4cm}cc|r}
\hline
\textbf{ID} &\textbf{Code Transformation} & \textbf{Repair Actions}%& \textbf{after} 
%& \textbf{Total(\%)}
\\ 
\hline
CT1&Conditional disposal of a resource
%& R1(16),R2(19),R3(9),R4(19),R5(7),R6(3),R8(1)
& R1,R2,R3,R4,R5,R6,R8
%& 29(6.8\%)
\\
CT2&Add call to dispose of function 
%& R1(17),R2(10),R3(9),R4(30),R5(12)
& R1,R2,R3,R4,R5
%& 42(9.8\%)
\\
CT3&Add dispose of function
%& R1(17),R2(2),R3(3),R4(8),R5(1),R7(1)
& R1,R2,R3,R4,R5,R7
%& 7(1.6\%)
\\
CT4&Set obsolete references to null 
%& R1(1),R2(3),R3(3),R4(4),R5(1)
& R1,R2,R3,R4,R5
%& 2(0.05\%)
\\
CT5&Add exception/try-exception construct
%& R1(4),R2(23),R5(5)
& R1,R2,R5
%& 41(9.6\%)
\\
CT6&Add finally/try-finally construct
%& R1(32),R2(42),R3(6),R4(6),R5(1),R6(1)
& R1,R2,R3,R4,R5,R6
%& 41(9.6\%)
\\
CT7&Use try-with-resource statement 
%& R1(3),R2(7),R3(1)
& R1,R2,R3
%&11(2.5\%)
\\
CT8&Change the condition arguments 
%& R1(3),R2(3),R4(2),R5(4)
& R1,R2,R4,R5
%& 29(6.8\%)
\\
CT9&Change method parameters 
%& R1(2),R2(2),R3(3),R4(3),R6(2),R7(4),R8(2)
& R1,R2,R3,R4,R6,R7,R8
%& 7(2\%)
\\
CT10&Change a static object to non-static 
%& R4(1),R7(1),R10(1)
& R4,R7,R10
%& 2(0.05\%)
\\
CT11&Change to weak reference
%& R8(4)
& R8
%& 1(0.02\%)
\\
CT12&Call another function
%& R1(1),R4(6),R6(1),R7(2)
& R1,R4,R6,R7
%& 5(1.2\%)
\\
CT13&Change to another collection 
%& R6(2), R7(3), R8(2)
& R6, R7, R8
%& 5(1.2\%)
\\
\hline
%\textbf{total} &&&&\textbf{164(38.3\%)}\\ \hline
\end{tabular}
\label{tab:actions-patterns}
\end{table*}

==> tables/table_defectLeak.tex <==
\begin{table}[t]
\centering
\caption{Detailed frequency of root causes in relationship with leak type. Column ``Conn.'' states numbers for connection leaks.}
\label{tab:defects_by_leakTypes}
\begin{tabular}{lrrrrr}
\hline 
\textbf{Defect} & \multicolumn{1}{l}{\textbf{Memory}} & \multicolumn{4}{c}{\textbf{Resources}}\\
\cline{3-6}
&  & \textbf{Total} & \textbf{File} & \textbf{Conn.} & \textbf{Thread}\\ 
\hline 
\emph{nonClosedRes} & - 		& \databars{57.9}{\%} 	& \databars{
53.2}{\%}  	& \databars{54}{\%}  	& \databars{71.2}{\%}\\ 
\emph{exception} 	& \databars{6.72}{\%} 	& \databars{33}{\%} 		& \databars{40.3}{\%} 	& \databars{36}{\%} 		& \databars{15.3}{\%} \\
\emph{collection} 	& \databars{39.07}{\%} 	&- 		& - 		& - 		& - \\
\emph{unrelRef} 	& \databars{23.95}{\%} 	&- 		& - 		& - 		& - \\
\emph{concurrency} 	& \databars{5.46}{\%} 	& \databars{2.1}{\%} 	& \databars{0.8}{\%} 	& \databars{6}{\%} 		& \databars{1.7}{\%} \\
\emph{schedule} 	& \databars{2.94}{\%} 	& \databars{3.4}{\%} 	& \databars{3.2}{\%} 	& \databars{2}{\%} 		& \databars{5.1}{\%} \\
\emph{cache} 		& \databars{5.88}{\%} 	& - 		& - 		& - 		& - \\
\emph{api} 			& \databars{3.7}{\%} 	& \databars{0.9}{\%} 	& \databars{0.8}{\%} 	& - 		& \databars{1.7}{\%} \\
%\emph{threadlocal} 	& \databars{3.7}{\%} 	& \databars{0.4}{\%} 	& \databars{0.8}{\%} 	& \databars{2}{\%} 		& - \\
\hline
\textbf{total} &\textbf{219} &\textbf{233} &\textbf{124} &\textbf{50} &\textbf{59} \\
\hline 
\end{tabular}
\end{table}
